Spike-based local synaptic plasticity: A survey of computational models and neuromorphic circuits

Understanding how biological neural networks carry out learning using spike-based local plasticity mechanisms can lead to the development of powerful, energy-efficient, and adaptive neuromorphic processing systems. A large number of spike-based learning models have recently been proposed following different approaches. However, it is difficult to assess if and how they could be mapped onto neuromorphic hardware, and to compare their features and ease of implementation. To this end, in this survey, we provide a comprehensive overview of representative brain-inspired synaptic plasticity models and mixed-signal CMOS neuromorphic circuits within a unified framework. We review historical, bottom-up, and top-down approaches to modeling synaptic plasticity, and we identify computational primitives that can support low-latency and low-power hardware implementations of spike-based learning rules. We provide a common definition of a locality principle based on pre- and post-synaptic neuron information, which we propose as a fundamental requirement for physical implementations of synaptic plasticity. Based on this principle, we compare the properties of these models within the same framework, and describe the mixed-signal electronic circuits that implement their computing primitives, pointing out how these building blocks enable efficient on-chip and online learning in neuromorphic processing systems.

==> community_feedback.tex <==
Community feedback

-------------------------------------

From: Jannes Jegminat
When: 04-11-2022

Lyes Khacef, thanks for the nice review!

Let me advertise two related Bayesian spiked-based plasticity models that I worked on during my Phd and that you might want to include.

We studied ideas how uncertainty can improve spike-based learning:

https://journals.plos.org/ploscompbiol/article/comments?id=10.1371/journal.pcbi.1009721

https://www.nature.com/articles/s41593-021-00809-5

-------------------------------------

From: Madison Cotteret -> DONE

Delta-dirac should be Dirac delta

-------------------------------------

From: Carver Mead -> DONE

> Hi Giacomo
> Thanks so much for getting in touch, and for the kind words.

[...]

>
> I looked at some of your pubs, and was particularly impressed by your review with Elisabetta Chicca arXiv2209.15536.
> I found a couple of typos: Top of p.4  ..."does requires"... delete does
> 2nd line p.6 - "let to" should be "led to"
>
> It was a particularly valuable synthesis of the neuro findings and the circuit work.

[...]

So it would be nice to add in the acknowledgments all the names of colleagues that provided feedback, including Carver's!

BTW, please make the corrections that he suggested.... 

-------------------------------------

From: Wouter Serdijn -> DONE
When: 27-10-2022

Dear all,

Wouter Serdijn (http://bioelectronics.tudelft.nl/~wout/ ) pointed out to Elisabetta that the bistability circuit of Fig.5 in our survey paper is wrong. The + and - terminals of the opamp should be swapped...

Can you please correct it. Add this sentence in the acknowledgments: "We thank Wouter Serdijn for fruitful discussions on circuit details." and upload a revised version to arxiv?

thanks, g.

-------------------------------------

From: Samuel R Schmidgall <sschmidg@gmu.edu>
When: 05-10-2022

Hello, Dr. Khacef.

I am extremely impressed by your review paper; it was very well written. I am a big fan of this work! I work on the algorithm side of plasticity for Neuromorphic systems and have always wanted to learn more about the circuit side, so this was a great read. 

The discussion on "6.2. Overcoming back-propagation limits for online learning” may benefit from the following papers of mine:

https://www.biorxiv.org/content/biorxiv/early/2022/06/28/2022.06.24.497562.full.pdf
https://www.frontiersin.org/articles/10.3389/fnbot.2021.629210/full

Where in these works, the interaction between a neuromodulatory signal and synaptic plasticity rule are optimized via gradient descent in a Neuromorphic system. I’d love to chat if you are interested in discussing this at all, or about plasticity in general.

Thank you,
Sam

---

It is a bit different but related to Neftci's, because most of the literature in plasticity designs a plasticity rule around some analytic equation (e.g. BPTT, or in this case MAML) but ours optimizes the plasticity rule to be best suited toward solving a particular set of problems using models of cortical plasticity taken from theoretical neuroscience literature instead of designing our own rules. In the first work I sent we optimized the plasticity rules to solve temporally-demanding online learning problems, and in both we showed significant adaptation outside of the task domain.

-------------------------------------

From: Ali Safa <LinkedIn>
When: 06-10-2022

Hi Lyes, 

Congratulations on your new job at Sony! If I remember correctly, we had a brief chat during your presentation at IMEC :-) 
Very interesting your new survey on STDP!! and very useful for the community. 
An emerging approach that I also find interesting is the top-down approaches "how to convert machine learning techniques into SNN-STDP". This one is excellent:
Neftci et al, "Event-driven contrastive divergence for spiking neuromorphic systems"

On our side, we have recently developed a new approach for STDP based on dictionary learning that outperforms the prior art on some DVS datasets:

https://ieeexplore.ieee.org/document/9892362

Here you go, I hope you'll find these refs interesting for the survey :-)

All the best,
Ali

Translated with www.DeepL.com/Translator (free version)

-------------------------------------

From: Sebastian Schmitt
When: 06-10-2022

Hi Lyes!
 
I've come across your latest preprint on plasticity in neuromorphic computing.
 
It's a nice overview! However, I'm a bit puzzled that you did not mention BrainScaleS.
 
I think it would be an important addition to your manuscript, as (programmable) plasticity is at the heart of it.
 
The best entry point is probably:
https://www.frontiersin.org/articles/10.3389/fnins.2022.795876/full
from which you'll find all the foundational publications.
 
Best,

Sebastian

---

Hi Sebastian,

thanks a lot! Actually, we did not mention BrainScaleS because we only reviewed dedicated analog circuits for real-time (as opposed to accelerated) emulation of synaptic plasticity. We will see how we can mention it and explain it clearly in the paper.

Thank you for your feedback!

Cheers,

Lyes.

-------------------------------------



==> meeting_minutes.tex <==
## 08.06.2021
Meeting with Lyes, Philipp, Arianna. 

- We include everything on the table and then remove things gradually
- 1997 paper by Misha, comes before the 2000, as an example of how building things are important
- We limit our research on analog rules on chip actually fabricated. REVERTED!!
- Include FPGA in table() Hamilto+ Tapson+ Van shaik , Frenkel) and then we will think about it. REVERTED!! 

- Other spreadsheet page for bio papers. (Eg Bi&Poo paper wit STDP synaptic observations)
- Look at Jennifer hassler work
- Implementation of Clopath work is mostly memristive
- Fusi rule paper before 2007?

# todo
- next meeting 18.6
- Finish table and Lyes will work on introduction


## 18.06.2021

Meeting with Lyes, Philipp, Arianna. 

-CMOS non digital hence mixed signal agreed with Elisabetta+Lyes+Philipp. Focus only on analog. FGAA can be included, because it is just Jennifer Hasler, and its analog.
-Keep clopath paper, even without memristive implementations

-Floating gate implementation not excluded

# todo
- next meeting 02.07
- Finish table for real 


## 02.07.2021

Meeting with Lyes, Philipp, Arianna. 

-Including FG not FPAA because its on a network level, instead of a synapse level
- Table is looking good. 
- Minor adjustments needed

#todo:
-Each get 1 model, write equations and variable table. We make it uniform later.
Next meeting 16.07


# 16.07.2021

-Rules are written
-Plans(i):Try and describe the basic components, and put them together for all rules, (ii) circuits of all implementations (iii) one circuit per rule and then different implementations

todo:
-In table just a generic A. and in explanation of rule A+/- A2/A3 e.g rename variables for consistency in table sigma and Ca variables represent Calcium
-Look at actual implementations of the circuits and discuss the diference and decide how to descibe circuits. Everyone does the ones they have done for the equations.

-Next meetings: 27.07 and 6.08


## 27.07.21
- Show only plasticity circuits
- Redraw the circuits and explain the main parts with colored boxes
- Clopat    h voltage-based rule: why is there no analog CMOS implementation?
- Deadline for proofreading by Elisabetta and Giacomo: 07/09/21.


## 06.08.21
- STDP paper = indiveri 2007
- TSTDP paper = azghadi 2013

- For next time add ~1/2 page per paper to describe rule and equations.
- For next time draw circuits for reference circuits 
- next meeting 3.09?


## 03.09.21
- separate the sections of modeling and implementation
- map the equation to the circuit blocks (show the transistors but not explain the full circuits)
- conclusion: come back to a higher level, wiring influences learning
- add transitions between paragraphs
- unify the learning rules
- references: please add them to biblio/new.bib

- ToDo:
* Philipp: Add Urbanzick-Senn rule + read the whole paper
* Arianna: Normalize (unify) the namings of the equations + read the whole paper
* Lyes: Add the table + introduction
* Matteo: Add the discussion/conclusion


## 10.09.21
- Circuits (Idea from Elisabetta): Draw the building blocks at the transistor level and briefly describe them in the caption of the figure, then simply use the building blocks for the learning circuits that are described at a the blocks level by linking the building boxes to the plasticity rules -> Describing at the transistor is too far for the scope of the paper. 

- What about reward STDP? -> non-local?

- Applications: depends on the network topology and could be discarded

- Length: is there any upper limit (pages)?

- Learning rules description: Urbenzick-Senn description is much longer than the others

- Urbenzicj-Senn: much closer to gradient-based learning as it explicitely minimizes an error signal (delta rule), should we keep it? 

- Normalizing the rules: use a table with common variables and small tables with detailed parameters for every rule

- Add a section for memristive implems

ToDo:
* Lyes: Complete the introduction  + reward STDP + PES rule + add the references of memristive implems for the Voltage-based STDP and RDSP
* Arianna: Add the common table and split the detailed table into the different rules + think about the possibility of having building blocks
* Philipp: Put the IOP latex format + vacation
* Matteo: Discussion


## 20.09.21

- Questions for Elisabetta and Giacomo:
* Learning rules: Keep the same equations as the original papers and add a table where we classify them to have the big picture?
* Circuits: Draw the circuit at the tansistor level, but describe it at the block level refering to the local variables in the rule itself - Readability?
* Title: maybe more broad on the modeling
* Learning rules: PES?

- Plan a meeting for mid-october: Doodle without Wednesdays

- Next meeting: Discuss the introduction

ToDo:
* Arianna and Matteo: Re-drawing circuits
* Philipp: Urbenzcik-Senn rule
* Lyes: Write the email + doodle, add the structural plasticity and complete the introduction


## 01.10.21
Questions for the meeting of 11.10:
- Short or long versions for the learning rules?
- Should we inbclude the circuits for Urbenczik from Dora and Ole's thesis?
- Discuss if/how to normalize the equations
- Brainstorm for the paper's title

ToDo:
* Lyes:
- Introduction: Have the gradient-based learning as a separate section?
- Historical perspective: Include Matteo's changes
- Answer Giacomo's comments

* Arianna:
- Send the email to Elisabetta and Giacomo for feedback on the circuits figures

* Matteo: new start for the introduction 

* Arianna, Matteo and Philipp
- Read the synaptic plasticity overview section for feedback

## 08.10.21
To discuss on monday:
- Rules to be added (filter = local + spike-based): hPES and BDSP -> OK
    - Filter should be ''implementable with existing CMOS circuits''
- If/how to normalize the equations: Pros and cons
    - Decision postponed until people have read the full ''rules part''
- How to describe the CMOS circuits
    - Describe CMOS implementations of computational primitives
    - For the existing ones, show block diagram maybe with chosen option inside
    - For the not existing ones, we show equation in colors or propose functional block diagram
- Length of rules description
    - Comparing the rules, using similar notations, short descriptions
- Section "Theoretical perspective" can be seen as redundant? Why it cannot be moved to the primitives section?
    - Section can stay if it shows the clear purpose of top-down
- WTA: need a full section?
    - Probably not??
- Make ''Computational primitives'' more clear to be ''synaptic plasticity computational primitives''
- Give more context about online learning? Which reference for hetero-synaptic competition?
- Paper's title: back to the first title

## 22.10.21
- Describe the circuits main components with text and references to the papers instead of figures
- Add Sadique Sheik rule
- Pawelzik rule?

## 11.11.21
- Text to present the CMOS primitives, then keep the original figures
- Normalization: no, we 

- Table 1: Lyes
    - Complete the table
    - Put the stop learning on *
    
- Table 3: Remove the applications and split the table into two tables

- Table 2: Add the missing columns -> Arianna, Matteo

- Matteo: Sheik rule

- Philpp: Graupner and Brunnel circuits + Saiek vs Pevelsik (homeostatic spiking vs homeostatic membrane potential)
- Philipp: Urbancyk/Senn:
- - No stop learning because backpropagated spike never causes zero error
- - postsynaptic dendritic voltage -> predicted postsynaptic voltage -> predicted postsynaptic spikerate

questions:
- do we write only the LR or also synapse/neuron model etc?


## 19.11.21
- Philpp: Graupner and Brunnel circuits
- Philipp: DPSS use PSP in equation
- Philipp: MPDP add variables table
- Philipp: Check variables and add rules in large variable table

-Highlight that the Hafliger et al 1997 paper implements ''STDP'' before it was formally described

## 26.11.21
- Make in the introduction clearer why we write the paper/content in the way we do.

- In introduction stress that there is a large variety of rules.


## 09.12.2021:
* Feedback from Elisabetta and Giacomo
- Introduction: revised by Elisabetta
- Historical plasticity: keep it?
- Rules:
    * table for common meaning of variables, uniformization by trigger
    * say why and what to make it shorter
- Circuits: put the elements in text
- Figures: proper caption
- Discussion and conclusion:
    * recover the focus on the circuit for the conclusion by discussing the differences on the circuits
    * better link of the model to the circuit -> local computing
- Comparing the models based on the circuits: if we only focus on area, we take STDP, but then we are limited on the application
- Adapting the title, examples of circuits, and their CMOS neuromorphic building blocks (primitives)
- Point out in the introduction the fact that local learning is different from back-prop
- Hafliger and Mahowald: RDSP? -> Ricatti
- Intro: by the end of the paper, you can decide how to choose a model -> do we?
- Better introduce the comparative tables
- Plan: Submission in February

## 21.01.2022
- Read the intro again and put the final comments (Lyes)
- Adapt the RDSP (Lyes) and DPSS + MPDP (Philipp)
- Define the "type" section of the circuits table

## 02.09.2022
- Split the work from Giacomo's feedback:
* Abstract     -> Lyes
* Introduction -> Lyes
* Overview     -> Lyes
* Primitives   -> Matteo
* Models       -> Philipp
* Circuits     -> Arianna
* Discussion   -> Everyone on her/his own section

## 09.09.2022
- About 50 comments to validate

==> new_plasticity_models.tex <==
Philipp: https://www.frontiersin.org/articles/10.3389/fnins.2022.983950/full

---

Lyes: https://arxiv.org/pdf/1807.10936.pdf
Lyes: https://www.biorxiv.org/content/10.1101/2022.10.26.513846v1
